Compositional Generalization from First Principles

Leveraging the compositional nature of our world to expedite learning and facilitate generalization is a hallmark of human perception. In machine learning, on the other hand, achieving compositional generalization has proven to be an elusive goal, even for models with explicit compositional priors. To get a better handle on compositional generalization, we here approach it from the bottom up: Inspired by identifiable representation learning, we investigate compositionality as a property of the data-generating process rather than the data itself. This reformulation enables us to derive mild conditions on only the support of the training distribution and the model architecture, which are sufficient for compositional generalization. We further demonstrate how our theoretical framework applies to real-world scenarios and validate our findings empirically. Our results set the stage for a principled theoretical study of compositional generalization.

==> 06_broader_impact.tex <==
\section*{Broader Impact}

==> compositional_ood_generalization/00_abstract.tex <==
Leveraging the compositional nature of our world to expedite learning and facilitate generalization is a hallmark of human perception. In machine learning, on the other hand, achieving compositional generalization has proven to be an elusive goal, even for models with explicit compositional priors. To get a better handle on compositional generalization, we here approach it from the bottom up: Inspired by identifiable representation learning, we investigate compositionality as a property of the data-generating process rather than the data itself. This reformulation enables us to derive mild conditions on only the support of the training distribution and the model architecture, which are sufficient for compositional generalization. We further demonstrate how our theoretical framework applies to real-world scenarios and validate our findings empirically. Our results set the stage for a principled theoretical study of compositional generalization.

==> compositional_ood_generalization/01_introduction.tex <==
\section{Introduction}\label{sec:intro}

% Compositional generalization, the ability to understand and extrapolate from known components to novel contexts by recombining them in new ways, is a cornerstone of human cognition and perception. It allows humans to drastically reduce learning complexity, promotes sample efficiency and facilitates generalization to novel inputs and tasks.

\textit{Systematic compositionality}~\cite{fodorConnectionismCognitiveArchitecture1988} is the remarkable ability to utilize a finite set of known components to understand and generate a vast array of novel combinations. This ability, referred to by Chomsky~\cite{chomsky2014aspects} as the ``\textit{infinite use of finite means}'', is a distinguishing feature of human cognition, enabling us to adapt to diverse situations and learn from varied experiences.

It's been a long-standing idea to leverage the compositional nature of the world for learning. In object-centric learning, models learn to isolate representations of individual objects as building blocks for complex scenes. In disentanglement, models aim to infer factors of variation that capture compositional and interpretable aspects of their inputs, for example hair color, skin color, and gender for facial data. So far, however, there is little evidence that these methods deliver substantially increased learning efficacy or generalization capabilities (\citet{schottVisualRepresentationLearning2022}, \citet{monteroRoleDisentanglementgeneralisation2022}). Across domains and modalities, machine learning models still largely fail to capture and utilize the compositional nature of the training data (\citet{lake2018generalization, loula2018rearranging, keysers2019measuring}).

% Consider the simple example of a scene containing two \textit{components}, in this case sprites with variable latent factors position, size, shape, and color. A simple multi-layer neural network can easily learn to reconstruct images with arbitrary \textit{compositions} of these sprites given each components' description. However, the model fails entirely to reconstruct images with unseen combinations of sprites---even if each such scene is merely a novel composition of previously observed components (Figure~\ref{fig:motivation}). Failure to generalize to unseen data in even this simplistic regression setting demonstrates that \textit{compositional generalization} does not automatically occur simply because the data seems to be of a compositional nature.

To exemplify this failure, consider a model trained on a data set with images of two sprites with varying position, size, shape, and color overlaid on a black canvas. Given the latent factors, a simple multi-layer neural network can easily learn to reconstruct images containing \textit{compositions} of these sprites that were covered by the training set (Figure~\ref{fig:motivation}, top rows). However, reconstruction fails for novel compositions---even if the individual \textit{components} have been observed before (Figure~\ref{fig:motivation}, bottom row). Failure to generalize to unseen data in even this simplistic regression setting demonstrates that \textit{compositional generalization} does not automatically emerge simply because the data is of a compositional nature.

We therefore take a step back to formally study compositionality and understand what conditions need to be fulfilled for compositional generalization to occur. To this end, we take inspiration from identifiable representation learning and define a broad class of data generating processes that are compositional and for which we can provably show that inference models can generalize to novel compositions that have not been part of the training set. More precisely, our contributions are as follows:
\begin{itemize}
    \item We specify \textit{compositional data-generating processes} both in terms of their function class and latent distributions (Sections~\ref{sec:compositionality} and \ref{sec:generalization}) such that they cover a wide range of assumptions made by existing compositional methods. %(e.g. Frady2023, SlotAttention, Complex-Valued AutoEncoder, ... \cite{}).
    
    \item We prove a set of sufficient conditions under which models trained on the data are able to generalize compositionally (Section~\ref{sec:conditions}).
    
    \item We validate our theory in a range of synthetic experiments and perform several ablation studies that relate our findings to empirical methods (Section~\ref{sec:experiments}).
\end{itemize}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{figs/fig1_motivation_v2.pdf}
  \caption{\textbf{Left}: We train a model $f$ to reconstruct images containing two sprites given their latent representation \texttt{(x, y, shape, size, color)}. \textbf{Center}: In the \textcolor{sbbluedeep}{\textbf{training set}} (top row and left column), one sprite is fixed in its base configuration (orange triangle or red circle), while the other can vary freely (in this example, sprite~1 varies in position, sprite~2 in shape and color). As a result, each sample in the \textcolor{sbreddeep}{\textbf{test set}} (lower right block) can be expressed as a novel \textit{composition} of known \textit{components}. \textbf{Right}: While the model is able to perfectly fit the training data, it fails to \textit{generalize compositionally} to the test data.}\label{fig:motivation}
\end{figure}

% \begin{itemize}
% \item long history of pushing for compositional models/representations (i.e. disentanglement)
% \item promise more interpretable methods, sample-efficient learning, similar representations to humans (e.g. object-centricity)
% \item we've seen that if compositionality is built in, it can be useful (e.g. compositional scenes in GIRAFFE)
% \item however, recent findings (Schott, Montero) show that compositionality does not simply arise from learning on compositional data, even with disentanglement priors
% \item therefore, we ask ourselves whether we can approach this from a theoretical angle: understand what compositional generalization is, and under what conditions it can occur
% \item specifically, since compositionality is a property of the data generating function, we want to understand this from a functional level, which is mostly independent of distributional assumptions
% \item this is different to other works on OOD generalization, which often look at distribution shifts or have strict assumptions on the distributions (e.g. First Steps ... paper)
% \item our contributions and outline of this paper
% \begin{itemize}
%     \item come up with theoretical framework/definitions that fit exisiting approaches (e.g. Frady2023, SlotAttention, Complex-Valued AutoEncoder, ...) \ref{sec:theory}
%     \item derive sufficient conditions for compositional generalization \ref{sec:theory}
%     \item show that there's a trade-off between inductive bias in the model and amount of data that needs to be observed?
%     \item conduct experiments that validate and demonstrate our setup
% \end{itemize}
% \end{itemize}



==> compositional_ood_generalization/02_related_work.tex <==
\section{Related Work}\label{sec:related}
\paragraph{Representation learning}
\textit{Disentanglement} and \textit{identifiable representation learning} aim to learn succinct representations that both factorize the data space efficiently and are robust towards distributional changes \cite{locatello2019fairness, 6472238, NEURIPS2019_bc3c4a63}. However, the expectation that more compositional representations lead to better out-of-distribution (OOD) generalization has not been met, as demonstrated by \citet{schottVisualRepresentationLearning2022} and \citet{monteroLostLatentSpace2022}. Although our work does not directly address generalization issues in identifiable representation learning, our setup is directly inspired by it, and we examine data-generating processes similar to \cite{reizinger2022embrace, zimmermann2021contrastive, von2021self}.

\paragraph{Empirical Approaches}
Many empirical methods use compositional priors and claim improved compositional generalization. The problem has been studied especially closely in language~\cite{russin2019compositional, akyurek2020learning, marcheggiani2018exploiting}, but it remains far from being solved~\cite{lake2018generalization, loula2018rearranging, keysers2019measuring}. Object-centric learning is another domain in which compositionality plays a major role, and many approaches explicitly model the composition of scenes from object-``slots''~\cite{locatelloObjectCentricLearningSlot2020, hinton2018matrix, greff2019multi, burgessMONetUnsupervisedScene2019, kipf2021conditional}. The slot approach is also common in vector-symbolic architectures like \cite{vankovTrainingNeuralNetworks2020} and \cite{fradyLearningGeneralizationCompositional2023}. For most of these works, however, compositional generalization is not a focal point, and their actual generalization capability remains to be studied. There are also some architectures like transformers~\cite{vaswaniAttentionAllYou2017}, graph neural networks~\cite{cappartcombinatorial}, bilinear models~\cite{hong2021bi}, or complex-valued autoencoders~\cite{loweComplexValuedAutoencodersObject2022} that have been claimed to exhibit some degree of compositional generalization, but again, principled analysis of their generalization ability is lacking. Our framework can guide the systematic evaluation of these methods. While we use the visual domain as an example throughout this work, our contributions are not tied to any specific data domain or modality. 

\paragraph{Theoretical approaches to OOD generalization}
The OOD generalization problem for non-linear models where train and test distributions differ in their densities, but not their supports, has been studied extensively, most prominently by \citet{ben2014domain} and \citet{sugiyama2007covariate}. We refer the reader to \citet{shenOutOfDistributionGeneralizationSurvey2021} for a comprehensive overview. In contrast, compositional generalization requires generalizing to a distribution with different, possibly non-overlapping support. This problem is more challenging and remains unsolved. \citet{ben2010theory} were able to show that models can generalize between distributions with a very specific relation, but it is unclear what realistic distributions fit their constraints. \citet{netanyahuLearningExtrapolateTransductive2023} also study \textit{out-of-support} problems theoretically but touch on compositional generalization only as a workaround for general extrapolation. Recently, \citet{dongFirstStepsUnderstanding2022} took a first step towards a more applicable theory of compositional generalization to unseen domains, but their results still rely on specific distributions, and they do not consider functions with arbitrary (nonlinear) compositions or multi-variate outputs. In contrast, our framework is independent of the exact distributions used for training and testing, and our assumptions on the compositional nature of the data allow us to prove generalization in a much broader setting. 

% To the best of our knowledge, Ben-David et al 2010, ,\citet{dongFirstStepsUnderstanding2022} and \citet{netanyahuLearningExtrapolateTransductive2023} are the three studies that examine the "Out-of-Support" generalization problem. In their work, Ben-David et al 2010 show that models can extrapolate from one distribution to another with a specific relation. Yet, it is unclear what realistic distributions fit these relational constraints. \citet{dongFirstStepsUnderstanding2022} lays some theoretical groundwork for extrapolating nonlinear models to unseen domains. Their results give a first indication that this could be theoretically achievable, but the application is limited by the reliance on specific distributions, and they only consider functions with complicated nonlinear compositions or multi-variate outputs. 

% DONT KNOW Where to mention this:
% There is a long history of trying to incorporate compositionality in machine learning models \cite{fodorConnectionismCognitiveArchitecture1988}. Yet it is unclear so far how symbolic information that allows for arbitrary recombination should be represented~\cite{greffBindingProblemArtificial2020}.

% \paragraph{Compositionality}
% There is a long history of trying to incorporate compositionality in machine learning models \cite{fodorConnectionismCognitiveArchitecture1988}.
% Yet it is unclear so far how symbolic information that allows for arbitrary recombination should be represented~\cite{greffBindingProblemArtificial2020}. A key expectation of disentangled representation learning, was that the these methods would aid generalization, especially compositional generalization, but this was shown to not be the case by both \citet{schottVisualRepresentationLearning2022} and \citet{monteroLostLatentSpace2022}.
% Some architectures, like transformers~\cite{vaswaniAttentionAllYou2017}, graph neural networks~\cite{cappartcombinatorial}, or bilinear models~\cite{hong2021bi} have been claimed to exhibit some degree of compositional generalization.
% Complex-valued autoencoders~\cite{loweComplexValuedAutoencodersObject2022} also seem to be able to compose multiple components to form a scene, but have not been examined in terms of their generalization performance.
% Unsupervised methods fail \cite{schottVisualRepresentationLearning2022, monteroRoleDisentanglementgeneralization2022} ...
% More Recently, many object-centric learning approaches like SlotAttention~\cite{locatelloObjectCentricLearningSlot2020} and many others~\cite{hinton2018matrix, greff2019multi, burgessMONetUnsupervisedScene2019, kipf2021conditional} explicitly compose scenes from multiple ``slots''. The slot approach is also common in vector-symbolic architectures like \cite{vankovTrainingNeuralNetworks2020} and \cite{fradyLearningGeneralizationCompositional2023}.
% \citet{fradyLearningGeneralizationCompositional2023} use a vector-symbolic architecture to learn compositional scene representations.

% \paragraph{OOD generalization}
% Compositional generalization falls under the umbrella of out-of-distribution generalization (see \citet{shenOutOfDistributionGeneralizationSurvey2021} for an overview) but makes stricter assumptions.
% In our case, which \citet{netanyahuLearningExtrapolateTransductive2023} term out-of-support generalization, the training and test distributions have different \textit{support}, not only varying \textit{densities}.
% This means works that study distributional robustness by bounding the difference to nearby distributions are less suited in this scenario.
% \citet{funkeDisentanglementGeneralizationCorrelation2022a} showed that even in supervised settings, generalization under just correlation shifts is challenging. It is not surprising, then, that out-of-support generalization can be tough even in the unsupervised case.
% \citet{madanWhenHowCNNs2021} investigate the problem empirically and reiterate that modular architectures can generalize better to unseen compositions.
% \citet{dongFirstStepsUnderstanding2022} lays some theoretical groundwork for extrapolating nonlinear models to unseen domains. Their results give a first indication that this could be theoretically achievable, but the application is limited by the reliance on specific distributions, and they only consider functions with complicated nonlinear compositions or multi-variate outputs. In contrast, our framework is independent of the exact distributions used for training and testing, and our assumptions on the compositional nature of the data allow us to prove generalization in a much broader setting.
% \citet{netanyahuLearningExtrapolateTransductive2023} also theoretically study out-of-support problems, but do not study compositions of multiple components.




% Overview of compositionality
% \begin{itemize}
%     \item History of papers pushing for compositionality/disentanglement
%     \item Main goal here: show it's an established concept, but there's not a lot of theoretical groundwork
% \end{itemize}

% Overview of (OOD) generalization
% \begin{itemize}
%     \item approaches that look at distributional assumptions
%     \item approaches/methods that claim generalization
%     \item connection/distinction of other types of generalization to compositional generalization
% \end{itemize}

% Compositional generalization
% \begin{itemize}
%     \item doesn't work out of the box (Schott, Montero)
%     \item distinction to the few related papers that look at this specific problem
% \end{itemize}

% define the terms ID, OOD here

==> compositional_ood_generalization/03_theory.tex <==
\section{A framework for compositional generalization}\label{sec:theory}
% The first part of this section explores how we can precisely capture our intuitive notion of compositionality. In the second part, we use this mathematical handle to derive sufficient conditions for compositional generalization to occur.

We use the following notation throughout. $[N]$ denotes the set of natural numbers $\{1, 2, ..., N\}$. $\boldsymbol{\mathrm {Id}}$~denotes the (vector-valued) identity function. We denote two functions $f, g$ agreeing for all points in set $P$ as $f {\equiv}_P \;g$. Finally, we write the total derivative of a vector-valued function $\boldsymbol f$ by all its inputs $\boldsymbol z$ as $\frac{\partial \boldsymbol f}{\partial \boldsymbol z}$, corresponding to the Jacobian matrix with entries $\frac{\partial f_i}{\partial z_j}$.

% $\boldsymbol J_{\boldsymbol f}(\boldsymbol x)$ denotes the Jacobian matrix of $\boldsymbol f$, i.e. $J_{f,ij} = \frac{\partial f_i}{\partial x_j}$.
% $a_i$ denotes the $i$-th component of the \emph{vector} or \emph{vector-valued function} $\boldsymbol a = \left(a_1, a_2, ...\right)^\top$.
% $a_{i,j}$ denotes the $j$-th element of the $i$-th vector in a \emph{vector of vectors} or \emph{vector of vector-valued functions} $\boldsymbol a = (\boldsymbol a_1, \boldsymbol a_2, ...), \boldsymbol a_1 = (a_{1,1}, a_{1,2}, ...)^\top$.
% $A_{i,j}$ denotes the element in row $i$ and column $j$ of \emph{matrix} $A$.



% \subsection{Compositional generalization as a property of the data-generating process}\label{sec:setup}

% To develop a more principled approach towards compositional generalization, we first have to formally define the terms \emph{compositionality} and \emph{generalization}.

% Before we can study conditions for compositional generalization, we need to refine our vague notion of what makes a dataset compositional in the first place. 

\subsection{Compositionality}\label{sec:compositionality}
% introduce running example
Colloquially, the term ``\emph{compositional data}'' implies that the data can be broken down into discrete, identifiable components that collectively form the whole. For instance, in natural images, these components might be objects, while in music, they might be individual instruments. As a running illustrative example, we will refer to a simple dataset similar to multi-dSprites~\cite{burgessMONetUnsupervisedScene2019}, as shown in Figure~\ref{fig:motivation}. Each sample in this dataset is a composition of two basic sprites, each with a random position, shape, size, and color, size.

% data generating process
Drawing inspiration from identifiable representation learning, we define compositionality mathematically as a property of the data-generating process. In our example, the samples are generated by a simple rendering engine that initially renders each sprite individually on separate canvases. These canvases are then overlaid to produce a single image featuring two sprites. More specifically, the rendering engine uses the (latent) properties of sprite one, $\boldsymbol z_1 = (z_{1,\text{x}}, z_{1,\text{y}}, z_{1,\text{shape}}, z_{1,\text{size}}, z_{1,\text{color}})$, to produce an image $\boldsymbol{\tilde x}_1$ of the first sprite. The same process is repeated with the properties of sprite two, $\boldsymbol z_2 = (z{2,\text{x}}, z_{2,\text{y}}, z_{2,\text{shape}}, z_{2,\text{size}}, z_{2,\text{color}})$, to create an image $\boldsymbol{\tilde x}_2$ of the second sprite. Lastly, the engine combines $\boldsymbol{\tilde x}_1$ and $\boldsymbol{\tilde x}_2$ to create the final overlaid rendering $\boldsymbol x$ of both sprites. Figure~\ref{fig:function_class} demonstrates this process.

In this scenario, the individual sprite renderers carry out the bulk of the work. In contrast, the composition of the two intermediate sprite images $\boldsymbol{\tilde x}_1, \boldsymbol{\tilde x}_2$ can be formulated as a simple pixel-wise operation (see Appendix~\ref{app:theory_details} for more details). The rendering processes for each sprite are independent: adjusting the properties of one sprite will not influence the intermediate image of the other, and vice versa.

% general definition of compositional data
We posit that this two-step generative procedure---the (intricate) generation of individual components and their (simple) composition into a single output---is a key characteristic of a broad class of compositional problems. If we know the composition function, then understanding the basic elements (for example, the individual sprites) is enough to grasp all possible combinations of sprites in the dataset.
% definition of a compositional representation
We can thus represent any latent variable model ${\boldsymbol f} : \mathcal{Z} \to \mathcal{X}$, which maps a latent vector ${\boldsymbol z}\in\mathcal{Z}$ to a sample $\boldsymbol x$ in the observation space $\mathcal{X}$, as a two-step generative process.

\begin{definition}[Compositional representation]\label{def:function_class}
$\{\boldsymbol C, \boldsymbol \varphi_1, \dots, \boldsymbol \varphi_K, \mathcal{Z}_1, \dots, \mathcal{Z}_K, \tilde{\mathcal{X}}_1, \dots, \tilde{\mathcal{X}}_K\}$ is a \textit{compositional representation} of function $\boldsymbol f$ if 
\begin{equation}
    \forall\boldsymbol{z}\in\mathcal{Z}\quad \boldsymbol f(\boldsymbol z) = \boldsymbol C \big( \boldsymbol \varphi_1(\boldsymbol z_1), ..., \boldsymbol \varphi_K(\boldsymbol z_K) \big)\quad\text{and}\quad\mathcal{Z} = \mathcal{Z}_1\times\dots\times\mathcal{Z}_K,
\end{equation}
where $\boldsymbol{z}_i$ denotes the canonical projection of $\boldsymbol{z}$ onto $\mathcal{Z}_i$. We refer to $\boldsymbol \varphi_k: \mathcal Z_k \to \tilde{\mathcal X}_k$ as the \textit{component functions}, to $\tilde{\mathcal X}_1, \dots, \tilde{\mathcal X}_K$ as the (hidden) component spaces, and to $\boldsymbol C: \tilde{\mathcal X}_1 \times \dots \times \tilde{\mathcal X}_K \to \mathcal X$ as the \textit{composition function}.
\end{definition}

Note that in its most general form, we do not require the component functions to be identical or to map to the same component space. The compositional representation of a function $\boldsymbol{f}$ is also not unique. For instance, any $\boldsymbol{f}$ possesses a trivial compositional representation given by $\{\boldsymbol{f}, \boldsymbol{\mathrm {Id}}, \dots, \boldsymbol{\mathrm {Id}}\}$ (for the sake of clarity, we will omit the explicit mention of the latent factorization and component spaces henceforth). We will later establish conditions that must be met by at least one compositional representation of $\boldsymbol{f}$.

% formal definition of compositional data
% In other words, we here define compositional data as being generated by a compositional latent variable model ${\boldsymbol f} : \mathbb{R}^L\to \mathbb{R}^O$ that maps a latent vector ${\boldsymbol z}\in\mathbb{R}^L$ to a sample $\boldsymbol x$ in the observation space $\mathbb{R}^O$ through a compositional function ${\boldsymbol f}$. We define compositionality of the mapping function ${\boldsymbol f}$ formally as follows using the idea of a two-step generative procedure:

% So far, we have referred to compositionality only in intuitive terms: Compositional data consists of multiple components; any number of components can be combined to form a specific data sample. This vague notion fits many domains and data modalities. In image data, even in simple scenes as the one in Figure~\ref{fig:motivation}, components could correspond to different objects. The composition of these can be as simple as arranging them in one joint scene, there does not need to be a complex interaction of components. In audio data, components could be individual signals, \eg individual speakers, which are simply overlaid to form novel combinations. But components could also interact in more complex ways. [COULDN'T THINK OF A GOOD EXAMPLE HERE]. The class of compositional data-generation processes needs to be broad enough to capture all of this.

% All of the examples have in common that we can split the data-generation process in two parts. First, there are \textit{component-wise generation processes}, which we will call \textit{slots}. The makeup of a scene consisting of a single component, \eg an image of a single object in front of a black background, would be solely governed by the generation process of this component, which takes its description as an input and outputs its representation. No matter how complex the interaction between components, there will be properties of each component that are independent of each other. Modifying one component won't change the other and vice-versa. These properties are modeled in each component slot. Components could share the same generation process, but do not need to.

% Second, there is the composition itself. Given all components, their interactions are modeled here. The output then is the data sample.

% If we allow the slot functions and the composition function to be arbitrary nonlinearities, we can model a \textit{compositional function} as depicted in Figure~\ref{fig:function_class} and formalized below.

\begin{figure}[t]
  \centering
  \begin{minipage}[b]{.425\textwidth}
      \centering
      \begin{adjustbox}{max width=\textwidth}
      \input{figs/function_class}
      \end{adjustbox}
      \vspace{8mm}
      \caption{\textit{Compositional representation} of a function (Definition~\ref{def:function_class}). \textit{Component functions} $\boldsymbol \varphi_k$ map each \textit{component latent} $\boldsymbol z_k$ to an intermediate representation $\boldsymbol{\tilde x}_k$. The \textit{composition function} $\boldsymbol C$ composes them into a final data point $\boldsymbol x$.}\label{fig:function_class}
  \end{minipage}%
  \hspace{.04\textwidth}
  \begin{minipage}[b]{.525\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/comp_support.pdf}
      \caption{\textbf{A-D} Distribution $P$ (blue) has \textit{compositional support} \wrt to the entire latent space if it has full support over the marginals. \textbf{E} Gaps in the support require the model to interpolate/extrapolate rather than generalize compositionally. \textbf{F} The support of the joint needs to be in an open set.}\label{fig:comp_support}
  \end{minipage}
\end{figure}

% \begin{definition}[Compositional function]\label{def:function_class}
% A function $\boldsymbol f$ is \textit{compositional} if it belongs to the function class $\mathcal F := \big\{\boldsymbol C \big( \boldsymbol \varphi_1(\boldsymbol z_1), ..., \boldsymbol \varphi_K(\boldsymbol z_K) \big) \big\} = \big\{ \boldsymbol C\big( \boldsymbol \varphi(\boldsymbol z) \big) \big\}$.
% The \textit{component functions} $\boldsymbol \varphi_k : \mathbb R^{D} \to \mathbb R^{M_k}$ map each \textit{slot latent} $\boldsymbol z_k$ to some intermediate representation $\boldsymbol{\tilde x}_k$.
% The \textit{composition function} $\boldsymbol C: \mathbb R^{K\times M} \to \mathbb R^N$ combines the outputs of all slot functions to the final output $\boldsymbol x$.
% In general, $N \geq M_k$.
% \end{definition}

 %This leaves a lot of leeway to view almost any function as compositional. and instead leave a more detailed this will get important once we derive under what conditions compositional generalization can occur.

% \begin{remark}
% In principle, each slot can have a different dimensionality, \ie $\boldsymbol z_k \in \mathbb R^{D_k}$, $\boldsymbol \varphi_k: \mathbb R^{D_k} \to \mathbb R^{M_k}$, and $\boldsymbol C: \mathbb R^K \times \mathbb R^{\sum_k M_k} \to \mathbb R^N$. For the sake of clarity, the following assumes $D_k = D$ and $M_k = M$ unless otherwise stated.
% \end{remark}

% connections to existing methods
Our definition of compositionality naturally aligns with various methods in the fields of identifiability, disentanglement, or object-centric learning. In the decoder of SlotAttention~\cite{locatelloObjectCentricLearningSlot2020}, for example, each component function is a spatial broadcast decoder followed by a CNN, and the composition function is implemented as alpha compositing.
%In contrast, complex-valued autoencoders~\cite{loweComplexValuedAutoencodersObject2022} distinguish the component functions by their phase while implementing the composition as a simple sum of complex-valued intermediate representations.
\citet{fradyLearningGeneralizationCompositional2023} model the component functions as element-wise multiplication of high-dimensional latent codes, which are then composed through a straightforward sum. A similar approach is chosen by \citet{vankovTrainingNeuralNetworks2020}, except that interactions between components are modeled using matrix multiplication. 


\subsection{Compositional Generalization}\label{sec:generalization}

The model in Figure~\ref{fig:motivation} was trained supervisedly, \ie it was trained to reconstruct samples $\boldsymbol{x}$ given the ground-truth latent factors $(\boldsymbol{z}_1, \boldsymbol{z}_2)$ for each sprite (see Section~\ref{sec:experiments} for more details). We denote this model as $\boldsymbol{\hat f}$, indicating that it is meant to replicate the ground-truth generating process $\boldsymbol{f}$ of the data. The model $\boldsymbol{\hat f}$ indeed learned to fit $\boldsymbol{f}$ almost perfectly on the training distribution $P$, but failed to do so on the test distribution $Q$.

This failure is surprising because the test samples only contain sprites already encountered during training. The novelty lies solely in the combination of these sprites. We would expect any model that comprehends the compositional nature of the dataset to readily generalize to these test samples.

This compositional aspect of the generalization problem manifests itself in the structure of the training and test distribution. In our running example, the model was trained on samples from a distribution $P$ that contained 
all possible sprites in each slot, but only in combination with one base sprite in the other slot (illustrated in Figure~\ref{fig:comp_support}A). More formally, the support of $P$ can be written as
\begin{equation}\label{eq:orthogonal}
    % \supp P = \left(\boldsymbol z_1 \in \mathcal Z_1, \boldsymbol z_2^0 \right) \cup \left(\boldsymbol z_1^0, \boldsymbol z_2 \in \mathcal Z_2 \right).
    \supp P = \left\{ (\boldsymbol z_1 \in \mathcal Z_1, \boldsymbol z_2 \in \mathcal Z_2) | \boldsymbol z_1 = \boldsymbol z_1^0 \vee \boldsymbol z_2 = \boldsymbol z_2^0 \right\}.
\end{equation}
The test distribution $Q$ is a uniform distribution over the full product space $\mathcal Z_1\times \mathcal Z_2$, i.e. it contains all possible sprite combinations. More generally, we say that a generalization problem is compositional if the test distribution contains only components that have been present in the training distribution, see Figure~\ref{fig:comp_support}. This notion can be formalized as follows based on the support of the marginal distributions:

% we can say that the support of the marginals of the two distributions should be the same, even if the support of the joint distribution differs. This is illustrated in Figure~\ref{fig:comp_support} and formalized below.

% introduce using running example
% In the running example from Figure~\ref{fig:motivation}, we loosely used the term \textit{generalization} to describe that the trained model should perform well on out-of-distribution data. We also refine this idea by looking at the data-generating process. In the example, the model was presented with samples in which only one of the objects was allowed to move from its origin configuration at a time. That is, the training set covered only a subset of the entire latent space , but omitted the large region of samples in which both objects differ from their origin configuration. The model, which we will call $\boldsymbol{\hat f}$, perfectly fit the data-generating process $\boldsymbol f$ on the training region of the latent space, but failed to do so on the larger test region. We can formalize the expectation we had on the model as follows:

% \begin{definition}[Generalization]\label{def:generalization}
% A function $\boldsymbol{\hat f}$ is said to \textit{generalize} from a training distribution $P$ to a test distribution $Q$ \wrt a ground-truth function $\boldsymbol f$, if agreement of both functions on $P$ implies agreement on $Q$, \ie
% \begin{equation}
%     \boldsymbol{\hat f} \underset{P}{\equiv} \boldsymbol f \implies \boldsymbol{\hat f} \underset{Q}{\equiv} \boldsymbol f.
% \end{equation}
% \end{definition}

% Note that the way we define generalization is particularly amenable to theoretical analysis: a function $\boldsymbol{\hat f}$ must generalize to $Q$ whenever it matches the ground-truth $\boldsymbol{f}$ on $P$. Put differently, we expect the learned model to generalize to out-of-domain (OOD) data whenever it performs perfectly on in-domain (ID) data.



% explain compositional support using running example
% Now, without further restriction on the relationship between $P$ and $Q$, there is little to say about whether or not a model can generalize. The reason why we expect the model in our running example to be able to generalize, is that it has already seen each individual sprite from the test set in its training distribution. The only novelty is the composition of sprites in the test images. This is the case because the training data was sampled from two orthogonal planes corresponding to
% \begin{equation}\label{eq:orthogonal}
%     \mathcal Z_\text{orthogonal} = \left(\boldsymbol z_1^0, \boldsymbol z_2 \in \mathcal Z_2 \right) \cup \left(\boldsymbol z_1 \in \mathcal Z_1, \boldsymbol z_2^0 \right),
%     % \mathcal Z_\text{orthogonal} = \left\{\boldsymbol z | \left(\boldsymbol z_1^0 \wedge \boldsymbol z_2 \in \mathcal Z_2\right) \vee \left(\boldsymbol z_1 \in \mathcal Z_1 \wedge \boldsymbol z_2^0\right) \right\}.
% \end{equation}
% where $\boldsymbol z_1^0, \boldsymbol z_2^0$ are the components' base configurations. This subset is illustrated in Figure~\ref{fig:comp_support}A. It is easy to see that if $Q$ is simply a distribution over $\mathcal Z_1 \times \mathcal Z_2$, choosing $\mathcal Z_\text{orthogonal}$ as the support for the training distribution $P$ should enable compositional generalization. More general, we can say that the support of the marginals of the two distributions should be the same, even if the support of the joint distribution differs. This is illustrated in Figure~\ref{fig:comp_support} and formalized below.

\begin{definition}[Compositional support]\label{def:comp_support}
Given two arbitrary distribution $P, Q$ over latents $\boldsymbol z = (\boldsymbol z_1, ..., \boldsymbol z_K) \in \mathcal Z = \mathcal Z_1 \times \cdots \times \mathcal Z_K$, $P$ has \textit{compositional support} \wrt $Q$ if
\begin{equation}
    % \supp P \subseteq \supp Q \subseteq \mathcal Z \quad\text{and}\quad 
    \supp P_{\boldsymbol z_k} = \supp Q_{\boldsymbol z_k} \subseteq \mathcal Z_k \quad\forall k \in [K].
\end{equation}
\end{definition}

% % explain support points, which are needed for the proof sketch
% A straightforward but important consequence of this definition is that a training distribution with compositional support will necessarily contain $K$ \textit{support points} $p^{k} \in P$ for each test latent $\boldsymbol q \in Q$. $\boldsymbol q$ can be composed from these support points as
% \begin{equation}
%     \boldsymbol q = (\boldsymbol q_1, ..., \boldsymbol q_K) = \left( \boldsymbol p_1^{1}, ..., \boldsymbol p_K^{K} \right).
% \end{equation}
% Additionaly, because the component functions are independent from each other, this is also true for the intermediate representations $\boldsymbol{\tilde x}_k = \boldsymbol \varphi(\boldsymbol z_k)$. They can similarly be expressed as
% \begin{equation}\label{eq:reconstruction}
%     \boldsymbol \varphi(\boldsymbol q) = \left( \boldsymbol\varphi_1 \left( \boldsymbol p_1^{1} \right), ..., \boldsymbol\varphi_K \left( \boldsymbol p_K^{K} \right) \right)
% \end{equation}
% This is illustrated in the left most column of Figure~\ref{fig:motivation}: We can find two training samples that contain the individual sprites to make up each test sample.

% compositional generalization
Clearly, \textit{compositional generalization} requires compositional support. If regions of the test latent space exist for which a component is not observed, as in Figure~\ref{fig:comp_support}E, we can examine a model's generalization capability, but the problem is not compositional. Depending on whether the gap in the support is in the middle of a latent's domain or towards either end, the generalization problem becomes an \textit{interpolation} or \textit{extrapolation} problem instead, which are not the focus of this work.


\subsection{Sufficient conditions for compositional generalization}\label{sec:conditions}
With the above setup, we can now begin to examine under what conditions compositional generalization can be guaranteed to occur.

To make this question precise, let us assume for the moment that the sprites don't occlude each other but that they are just summed up in pixel space. Then the compositional representation of the generative process is simply $\{\boldsymbol{\mathrm {Id}}, \boldsymbol{\varphi}_1, \boldsymbol{\varphi}_2\}$, i.e.
\begin{equation}
    \label{eq:sumcase}
    \boldsymbol{f}(\boldsymbol{z}) = \boldsymbol{\varphi}_1(\boldsymbol z_1) + \boldsymbol{\varphi}_2(\boldsymbol z_2).
\end{equation}

The question becomes: Given supervised samples $(\boldsymbol{z}_i, \boldsymbol{x}_i)$ from $P$, can we learn a new model $\boldsymbol{\hat f}$ that is equivalent to $\boldsymbol{f}$ on $Q$, i.e. for which $\boldsymbol{\hat f}\equiv_{Q} \boldsymbol{f}$? We assume that $\boldsymbol{C}$ is known, so in order to generalize, we must be able to reconstruct the individual component functions $\boldsymbol{\varphi}_i$.

For the simple case from equation~\ref{eq:sumcase}, we can fully reconstruct the component functions as follows. First, we note that if $\supp P$ is in an open set, we can locally reconstruct the hidden Jacobian of $\boldsymbol{\varphi}_i$ from the observable Jacobian of $\boldsymbol{f}$ as
\begin{equation}
    \frac{\partial\boldsymbol{f}}{\partial\boldsymbol{z}_k}(\boldsymbol{z}) = \frac{\partial\boldsymbol{\varphi}_k}{\partial\boldsymbol{z}_k}(\boldsymbol{z}_k).
\end{equation}
Since the training distribution contains all possible component configurations $\boldsymbol{z_i}$, we can reconstruct the Jacobian of $\boldsymbol{\varphi_i}$ in every point $\boldsymbol{z_i}$. Then we know everything about $\boldsymbol{\varphi_i}$ up to a global offset (which can be removed if there exists a known initial point for integration).

% If our training distribution has compositional support (see ...), then we can fully reconstruct the output of each component function $\boldsymbol{\varphi}_i$ for all possible component configurations. In turn, this allows us to provably generalize to all possible component combinations.

Our goal is to extend this approach to a maximally large set of composition functions $\boldsymbol{C}$. Our reasoning is straightforward if $\boldsymbol{C}$ is the identity, but what if we have occlusions or other nonlinear interactions between slots? What are general conditions on $\boldsymbol{C}$ and the support of the training distribution $P$ such that we can still reconstruct the individual component functions and thus generalize compositionally?

Let us now consider the sprites example with occlusions, and let us assume that the support of $P$ is basically a thin region around the diagonal; see Figure~\ref{fig:suff_support}~(left). In this case, the two sprites are always relatively similar, leading to large overlaps. It is impossible to reconstruct the full Jacobian of the occluded sprite from a single sample. Instead, we need a set of samples for which the background sprite is the same while the foreground sprite is in different positions; see Figure~\ref{fig:suff_support}~(right). With sufficient samples of this kind, we can observe all pixels of the background sprite at least once. Then reconstruction of the Jacobian of $\boldsymbol{\varphi_1}$ is possible again.

This line of thought brings us to a more general condition on the data-generating process: The composition function $\boldsymbol{C}$ and the support $P$ must be chosen such that the full Jacobian can be reconstructed for each component function for all component latents. We formally define the concept of \emph{sufficient support} below. Note that whether the support of $P$ is sufficient or not strongly depends on the choice of composition function $\boldsymbol{C}$.

% To answer this, we need to look at one aspect of the dataset above that we have glossed over so far: occlusions. The statement from section~\ref{sec:generalization} that we can compose each test sample from parts of the training samples is only true in the absence of sprites occluding parts of each other. This is illustrated in Figure~\ref{fig:suff_support}~(left): If we assume an orthogonal training support as before and have sprite~1 render in front of sprite~2, then there will necessarily be parts of the latent space for which perfect reconstruction of sprite~2 is impossible. Only if we observe enough points completely reason about the full appearance of sprite~2 for this latent value (Figure~\ref{fig:comp_support}~right) can we confidently argue that reconstruction should be possible.

% More generally, the assumption here is that the training support needs to be chosen broad enough such that the full information required for reconstruction in each latent value can be observed. How broad the support needs to be depends on the composition function. If the sprites in our example were overlaid transparently, the simple orthogonal support would clearly be sufficient.

% The relationship between the composition function and the support can be modeled by considering the derivative of the composition function with respect to the intermediate representation of each component. Only if a change to the component representation is also observable in the output (and thus the derivative is non-zero) can the reconstruction be successful. Since this needs to be fulfilled for all components in all output dimensions, we end up with a rank condition on the Jacobian matrix of the composition function, which we formally state below.

\begin{definition}[Sufficient support]\label{def:suff_support}
A distribution $P$ over latents $\boldsymbol z = (\boldsymbol z_1, ..., \boldsymbol z_K) \in \mathcal Z$, has \textit{sufficient support} \wrt a compositional representation of a function $\boldsymbol f$, if $\supp P$ is in an open set and for any latent value $\boldsymbol z_k^*$, there exists a (finite) set of points $P'_k(\boldsymbol z_k^*) \subseteq \{\boldsymbol p \in \supp P| \boldsymbol p_k = \boldsymbol z_k^* \}$ for which the sum of total derivatives of $\boldsymbol C$ has full rank. That is,
\begin{equation}
    \rank \sum_{\boldsymbol p \in P'_k(\boldsymbol z_k^*)} \frac{\partial \boldsymbol C}{\partial \boldsymbol \varphi_k}\big(\boldsymbol \varphi(\boldsymbol p)\big) = M,
\end{equation}
where $M$ is the dimension of the component space $\mathcal{\tilde X}_k \subseteq \mathbb R^M$.
\end{definition}

We are now ready to state our main theorem, namely that if $\boldsymbol{f}, \boldsymbol{\hat f}$ share the same composition function and if $P$ has compositional and sufficient support, then the model $\boldsymbol{\hat f}$ generalizes to $Q$ if it matches the ground-truth data-generating process $\boldsymbol{f}$ on $P$.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/suff_support.pdf}
  \caption{Illustration of the \textit{sufficient support} condition. For a (compositional) diagonal support, all samples will contain sprites with similar positions, leading to heavy occlusions and making reconstruction of the background sprite impossible (left). Reconstruction of the background sprite is only possible if the support is chosen broad enough, such that the subset of points sharing the same background sprite $P'$ contains samples with sufficient variance in the foreground sample. Specifically, each pixel of the background sprite must be observable at least once (right).}\label{fig:suff_support}
\end{figure}

\begin{theorem}\label{theorem}
Let  $P$, $Q$ be arbitrary distributions over latents $\boldsymbol z = (\boldsymbol z_1, ..., \boldsymbol z_K) \in \mathcal Z$.
Let $\boldsymbol f, \boldsymbol{\hat f}$ be functions with \emph{compositional representations} in the sense of definition~\ref{def:function_class} that share $\{ \boldsymbol C, \mathcal Z_1, ..., \mathcal Z_K \}$, but use arbitrary $\{ \boldsymbol{\varphi}_1, ..., \boldsymbol{\varphi}_K, \mathcal{\tilde X}_1, ..., \mathcal{\tilde X}_K \}, \{ \boldsymbol{\hat\varphi}_1, ..., \boldsymbol{\hat\varphi}_K, \mathcal{\hat X}_1, ..., \mathcal{\hat X}_K \}$.

Assume the following assumptions hold:
\begin{enumerate}[label=(A\arabic*)]
    \item\label{ass:well_behaved} $\boldsymbol C, \boldsymbol \varphi_k, \boldsymbol{\hat \varphi}_k$ are differentiable, $\boldsymbol C$ is Lipschitz in $\boldsymbol\varphi$, and $\boldsymbol\varphi$ is continuous in $\boldsymbol z$.
    \item\label{ass:comp_support} $P$ has \emph{compositional support} \wrt $Q$ in the sense of definition~\ref{def:comp_support}.
    \item\label{ass:suff_support} $P$ has \emph{sufficient support} \wrt $\boldsymbol f$ in the sense of definition~\ref{def:suff_support}.
    \item\label{ass:initial_point} There exists an initial point $\boldsymbol p^0\in \supp P$ such that $\boldsymbol \varphi (\boldsymbol p^0) = \boldsymbol{\hat \varphi}(\boldsymbol p^0)$.
\end{enumerate}

Then $\boldsymbol{\hat f}$ generalizes to $Q$, \ie $\boldsymbol f \underset{P}{\equiv} \boldsymbol{\hat f} \implies \boldsymbol f \underset{Q}{\equiv} \boldsymbol{\hat f}$.
\end{theorem}

The proof follows roughly the intuition we developed above in that we show that the Jacobians of the component functions can be reconstructed everywhere. Bear in mind that this is simply a construction for the proof: The theorem holds whenever $\boldsymbol{\hat f}$ fits the output of $\boldsymbol{f}$ on the training distribution $P$, which we can achieve with standard supervised training and without access to the ground-truth Jacobians. It should also be emphasized that since the compositional representation is not unique, the theorem holds if there exists at least one for which the assumptions are fulfilled. Note also that the initial point condition \ref{ass:initial_point} is needed in the proof, but in all practical experiments (see below), we can generalize compositionally without explicit knowledge of that point. We relegate further details to Appendix~\ref{app:proof}.

% \paragraph{Proof Sketch} We present a quick overview of the proof for theorem~\ref{theorem} here and give a brief intuition about the minor additional assumptions. The full proof is in appendix~\ref{app:proof}. Since we assume the same $\boldsymbol C$ for both functions, we only need to prove that $\boldsymbol f \underset{P}{\equiv} \boldsymbol{\hat f}$ implies $\boldsymbol \varphi \underset{Q}{\equiv} \boldsymbol{\hat \varphi}$. Since $P$ has compositional support, we know we can reconstruct the component function output on $Q$ from the support points in $P$ (Equation~\ref{eq:reconstruction}, and therefore only require agreement on $P$. This essentially amounts to trying to invert $\boldsymbol C$, which is not guaranteed to be possible globally. For example in the presence of occlusions, this will not be the case. Instead, we can show that if $P$ has sufficient support, we can (locally) uniquely solve for the derivatives of the component functions, such that we get $\frac{\partial\boldsymbol\varphi}{\partial\boldsymbol z} \underset{P}{\equiv} \frac{\partial\boldsymbol{\hat\varphi}}{\partial\boldsymbol z}$. To get agreement of the component functions themselves, all we require is that there exists some initial point in $P$ for which the component functions of the ground truth and model agree (Assumption~\ref{ass:initial_point}).



==> compositional_ood_generalization/04_experiments.tex <==
\section{Experiments}\label{sec:experiments}
We validate our theoretical framework on the multi-sprite data. All models were trained for 2000 epochs on training sets of 100k samples using an NVIDIA\,RTX\,2080\,Ti; all test sets contain 10k samples. Table~\ref{tab:experiments} summarizes the reconstruction quality achieved on the in-domain (ID) test set ($P$) and the entire latent space ($Q$) for all experiments.

\paragraph{Motivating experiment}\label{sec:main_experiment}
We implement the setup from Figure~\ref{fig:motivation} to demonstrate that a compositional model does indeed generalize if the conditions from Theorem~\ref{theorem} are met. We model the component functions as four fully-connected layers followed by four upsampling-convolution stages, mapping the 5d component latent to $64\times64$ RGB images. For training stability, the composition function is implemented as a soft pixel-wise addition using the sigmoid function $\sigma(\cdot)$ as
\begin{equation}\label{eq:add_sigmoid}
    \boldsymbol x = \sigma(\boldsymbol{\tilde x}_1) \cdot \boldsymbol{\tilde x}_1 + \sigma(-\boldsymbol{\tilde x}_1) \cdot \boldsymbol{\tilde x}_2,
\end{equation}
which allows component~1 to occlude component~2. We contrast this to a non-compositional \textit{monolithic} model, which has the same architecture as a single component function (with adjusted layer sizes to match the overall parameter count of the compositional model). We show that both models have the capacity to fit the data by training on random samples covering the entire latent space (Table~\ref{tab:experiments}, \textbf{\#1,2}). We then train on a distribution with orthogonal support as in equation~\ref{eq:orthogonal}, albeit with two planes for the foreground component to satisfy the sufficient support condition (Definition~\ref{def:suff_support}) as explained in Figure~\ref{fig:suff_support}. Both models can reconstruct ID samples, but only the compositional model generalizes to the entire latent space (Table~\ref{tab:experiments}, \textbf{\#3,4}).


% The ID set illustrated in Figure~\ref{fig:motivation} is an orthogonal set as in Equation~\ref{eq:orthogonal}, albeit with two planes for the first component which is rendered in front to satisfy the sufficient support condition (Definition~\ref{def:suff_support}) as explained in Figure~\ref{fig:suff_support}. The base configurations for component one are a small red circle in the top right corner and a small cyan square in the center, the base configuration for component two is a small orange triangle in the bottom left. We show that a compositional model, which implements the component functions as four full-connected layers, followed by four upsampling-convolution stages has no problem generalizing to the entire latent space when trained on the orthogonal training set. In contrast, the monolithic (non-compositional) model used in Figure~\ref{fig:motivation}, which uses the same architecture as a single component function (with adjusted layer sizes to math the overall parameter count of the compositional model) fits the ID data perfectly, but fails OOD. We compare to training on random samples covering the entire latent space to demonstrate that both models have the capacity to fit the data in principle.

\begin{table}[t]
    \centering
    \sisetup{
        tight-spacing=true,
        detect-family=true,
        detect-weight=true,
        mode=text,
        output-exponent-marker=\text{e}
    }
    \setlength{\tabcolsep}{0.4em}
    \renewcommand{\bfseries}{\fontseries{b}\selectfont} 
    \newrobustcmd{\B}{\bfseries}
    \begin{tabular}{r l l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.3] @{\hspace{1pt}} l S[table-format=-1.3] @{\hspace{1pt}} l }
        \toprule
        \B \# & \B Train Set & \B Model & \multicolumn{2}{c}{\B MSE ID $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B MSE all $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B $R^2$ ID $\scriptstyle\uparrow$} & \multicolumn{2}{c}{\B $R^2$ all $\scriptstyle\uparrow$} \\
        \midrule
         1 & Random     & Monolithic    & 1.73e-3 & \sd{1.47e-05} & 1.73e-3 & \sd{1.47e-05} & 0.931 & \sd{5.75e-04} & 0.931 & \sd{5.83e-04} \\
         2 & Random     & Compositional & 1.07e-03 & \sd{2.57e-05} & 1.07e-03 & \sd{2.57e-05} & 0.957 & \sd{1.02e-03} & 0.957 & \sd{1.02e-03} \\
         3 & Orthogonal & Monolithic    & 8.49e-04 & \sd{2.89e-05} & 4.06e-02 & \sd{3.86e-03} & 0.948 & \sd{1.71e-03} & -0.500 & \sd{6.70e-02} \\
         4 & Orthogonal & Compositional & 6.94e-04 &	\sd{1.09e-05} &	1.24e-03 &	\sd{4.11e-05} &	0.957 &	\sd{6.41e-04} &	0.951 &	\sd{1.43e-03}\\
        \midrule
         5 & Ortho.$\sim\mathcal N$ & Compositional & 7.01e-04 &	\sd{8.69e-06} &	1.24e-03 &	\sd{2.56e-05} &	0.957 &	\sd{5.51e-04} &	0.951 &	\sd{1.00e-03} \\
         6 & Diagonal & Compositional & 8.87e-04 &	\sd{1.03e-04} &	1.39e-03 &	\sd{4.04e-04} &	0.954 &	\sd{5.39e-03} &	0.945 &	\sd{1.61e-02} \\
        % \midrule
         7 & Ortho. (broad) & Compositional & 6.50e-04 &	\sd{1.52e-05} &	1.16e-03 &	\sd{3.32e-05} &	0.959 &	\sd{9.67e-04} &	0.954 &	\sd{1.31e-03} \\
         8 & Diag. (broad) & Compositional & 9.51e-04 &	\sd{2.78e-05} &	1.13e-03 &	\sd{3.10e-05} &	0.957 &	\sd{1.24e-03} &	0.955 &	\sd{1.23e-03} \\
        \midrule
        % Orthogonal bad support & 6.87e-04 &	\sd{4.99e-06} &	3.29e-03 &	\sd{2.27e-04} &	0.954 &	\sd{3.40e-04} &	0.869 &	\sd{9.06e-03} \\
         9 & Ortho. (gap) & Compositional & 7.36e-04 &	\sd{2.70e-05} &	2.64e-03 &	\sd{1.81e-04} &	0.954 &	\sd{1.68e-03} &	0.895 &	\sd{7.40e-03} \\
        10 & Diag. (narrow) & Compositional & 2.22e-03 &	\sd{1.24e-03} &	1.04e-02 &	\sd{7.10e-03} &	0.867 &	\sd{7.45e-02} &	0.589 &	\sd{2.82e-01} \\
        % \midrule
        11 & Orthogonal & Comp. (RGBa) & 2.67e-04 &	\sd{2.81e-06} &	5.24e-04 &	\sd{3.68e-06} &	0.984 &	\sd{1.80e-04} &	0.979 &	\sd{1.44e-04}\\
        \bottomrule
    \end{tabular}
    \vspace{10pt}
    \caption{We report the reconstruction quality measured as mean squared error (MSE, lower is better) and variance-weighted $R^2$ score (closer to 1 is better) for both the in-domain (ID) test set and the entire latent space, averaged over 5 random seeds. \textbf{\#1-4} The results demonstrate that a \textit{monolithic} model fails to generalize in the setup from Figure~\ref{fig:motivation}, but a \textit{compositional} model performs well on the entire latent space. \textbf{\#5-8} Generalization can occur in a variety of settings that fulfill the sufficient conditions from Theorem~\ref{theorem}. \textbf{\#9,10} Violating the compositional and sufficient support condition prohibits generalization, while choosing a more complex function class still works (\textbf{\#11}).}\label{tab:experiments}
\end{table}

% \begin{table}[t]\label{tab:main_experiment}
%     \centering
%     \sisetup{
%         tight-spacing=true,
%         detect-family=true,
%         detect-weight=true,
%         mode=text,
%         output-exponent-marker=\text{e}
%     }
%     \setlength{\tabcolsep}{0.4em}
%     \renewcommand{\bfseries}{\fontseries{b}\selectfont} 
%     \newrobustcmd{\B}{\bfseries}
%     \begin{tabular}{l l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.3] @{\hspace{1pt}} l S[table-format=-1.3] @{\hspace{1pt}} l }
%         \toprule
%         \B Train Set & \B Model & \multicolumn{2}{c}{\B MSE ID $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B MSE all $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B $R^2$ ID $\scriptstyle\uparrow$} & \multicolumn{2}{c}{\B $R^2$ all $\scriptstyle\uparrow$} \\
%         \midrule
%         Random     & Monolithic    & 1.73e-3 & \sd{1.47e-05} & 1.73e-3 & \sd{1.47e-05} & 0.931 & \sd{5.75e-04} & 0.931 & \sd{5.83e-04} \\
%         Random     & Compositional & 1.07e-03 & \sd{2.57e-05} & 1.07e-03 & \sd{2.57e-05} & 0.957 & \sd{1.02e-03} & 0.957 & \sd{1.02e-03} \\
%         Orthogonal & Monolithic    & 8.49e-04 & \sd{2.89e-05} & 4.06e-02 & \sd{3.86e-03} & 0.948 & \sd{1.71e-03} & -0.500 & \sd{6.70e-02} \\
%         Orthogonal & Compositional & 6.94e-04 &	\sd{1.09e-05} &	1.24e-03 &	\sd{4.11e-05} &	0.957 &	\sd{6.41e-04} &	0.951 &	\sd{1.43e-03}\\
%         \bottomrule
%     \end{tabular}
%     \vspace{10pt}
%     \caption{Reconstruction quality of a compositional and monolithic model. Given a compositional support, the monolithic model fails to generalize to unseen combinations (columns "all", see also Figure~\ref{fig:motivation}), while the compositional model still generalizes to the entire domain.}
% \end{table}



% \subsection{Ablations}\label{sec:ablations}
% We ablate multiple design choices in the implementation of the training setting and compositional model in Table~\ref{tab:ablations} to illustrate the main points of the theory.

\paragraph{Flexible compositional support} Next, we demonstrate the variety of settings that fulfil the compositional support assumption as illustrated in Figure~\ref{fig:comp_support}B and C. To this end, we repeat the experiment on training sets $P$ sampled from (i) a normal distribution with orthogonal support (Table~\ref{tab:experiments}, \textbf{\#5}) and (ii) a uniform distribution over a diagonal support chosen broad enough to satisfy the sufficient support condition (Table~\ref{tab:experiments}, \textbf{\#6}). The model generalizes to the entire latent space in both settings. Since the generalization performance is already close to ceiling, broadening the support of both distributions (Table~\ref{tab:experiments}, \textbf{\#7,8}) does not further increase performance.

\paragraph{Violating Conditions} Finally, we look at the effect of violating some conditions.

\begin{itemize}[leftmargin=12pt]
    \item \textbf{Gaps in support} (Table~\ref{tab:experiments}, \textbf{\#9}) If there are gaps in the support of the training set such that some component configurations are never observed (Figure~\ref{fig:comp_support}E) violates the compositional support condition (Definition~\ref{def:comp_support}). While the overall reconstruction performance only drops slightly, visualizing the reconstruction error over a 2d-slice of the latent space in Figure~\ref{fig:heatmap} illustrates clearly that generalization fails exactly where the condition is violated.
    
    \item \textbf{Insufficient training variability} (Table~\ref{tab:experiments}, \textbf{\#10}) Reducing the width of the diagonal support violates the sufficient support condition (Definition~\ref{def:suff_support}) as soon as some parts of the background component are always occluded and can not be observed in the output anymore. We can clearly see that reconstruction performance on the entire latent space drops significantly as a result.
    
    \item \textbf{Collapsed Composition Function} (Table~\ref{tab:experiments}, \textbf{\#11}) Changing the output of each component function from RGB to RGBa and implementing the composition as alpha compositing yields a model that is still compositional, but for which no support can satisfy the sufficient support condition since the derivative of transparent pixels will always be zero and the Jacobian matrix can therefore never have full rank (more details in Appendix~\ref{app:theory_details}). However, we observe that the model still generalizes to the entire latent space and achieves even lower reconstruction error than the original model. This emphasizes that what we present are merely \textit{sufficient} conditions, which might be loosened in future work.
\end{itemize}

% \begin{wrapfigure}{R}{0.6\textwidth}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/heatmap_annotated.pdf}
    \caption{Heatmap of the reconstruction error over a $z_{1,\text{x}}$-$z_{2,\text{x}}$-projection of the latent space with overlaid training support (red). Generalization can occur when the support is compositional (left) but fails exactly where the support is incomplete at $z_{1,\text{x}} \in [0.14, 0.46]$ (right).}\label{fig:heatmap}
\end{figure}
% \end{wrapfigure}

% (Table~\ref{tab:experiments}\#9) Introducing a gap in the support of the training set over $z_{1, \text{x}}$ such that component~1 is never observed with $x$-coordinates $[0.14..0.46]$ violates the compositional support condition (Definition~\ref{def:comp_support}).  

% \begin{table}[t]\label{tab:ablations}
%     \centering
%     \sisetup{
%         tight-spacing=true,
%         detect-family=true,
%         detect-weight=true,
%         mode=text,
%         output-exponent-marker=\text{e}
%     }
%     \setlength{\tabcolsep}{0.4em}
%     \renewcommand{\bfseries}{\fontseries{b}\selectfont} 
%     \newrobustcmd{\B}{\bfseries}
%     \begin{tabular}{l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.2e-1] @{\hspace{1pt}} l S[table-format=1.3] @{\hspace{1pt}} l S[table-format=1.3] @{\hspace{1pt}} l }
%         \toprule
%         \B Ablation & \multicolumn{2}{c}{\B MSE ID $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B MSE all $\scriptstyle\downarrow$} & \multicolumn{2}{c}{\B R² ID $\scriptstyle\uparrow$} & \multicolumn{2}{c}{\B R² all $\scriptstyle\uparrow$} \\
%         \midrule
%         -- & 6.94e-04 &	\sd{1.09e-05} &	1.24e-03 &	\sd{4.11e-05} &	0.957 &	\sd{6.41e-04} &	0.951 &	\sd{1.43e-03}\\
%         \midrule
%         Orthogonal $\sim\mathcal N(0.5, 1)$ & 7.01e-04 &	\sd{8.69e-06} &	1.24e-03 &	\sd{2.56e-05} &	0.957 &	\sd{5.51e-04} &	0.951 &	\sd{1.00e-03} \\
%         Diagonal 0.1 & 8.87e-04 &	\sd{1.03e-04} &	1.39e-03 &	\sd{4.04e-04} &	0.954 &	\sd{5.39e-03} &	0.945 &	\sd{1.61e-02} \\
%         % \midrule
%         Orthogonal larger support & 6.50e-04 &	\sd{1.52e-05} &	1.16e-03 &	\sd{3.32e-05} &	0.959 &	\sd{9.67e-04} &	0.954 &	\sd{1.31e-03} \\
%         Diagonal larger support & 9.51e-04 &	\sd{2.78e-05} &	1.13e-03 &	\sd{3.10e-05} &	0.957 &	\sd{1.24e-03} &	0.955 &	\sd{1.23e-03} \\
%         \midrule
%         % Orthogonal bad support & 6.87e-04 &	\sd{4.99e-06} &	3.29e-03 &	\sd{2.27e-04} &	0.954 &	\sd{3.40e-04} &	0.869 &	\sd{9.06e-03} \\
%         Orthogonal gap & 7.36e-04 &	\sd{2.70e-05} &	2.64e-03 &	\sd{1.81e-04} &	0.954 &	\sd{1.68e-03} &	0.895 &	\sd{7.40e-03} \\
%         Diagonal 0.05 & 2.22e-03 &	\sd{1.24e-03} &	1.04e-02 &	\sd{7.10e-03} &	0.867 &	\sd{7.45e-02} &	0.589 &	\sd{2.82e-01} \\
%         % \midrule
%         Alpha compositing & 2.67e-04 &	\sd{2.81e-06} &	5.24e-04 &	\sd{3.68e-06} &	0.984 &	\sd{1.80e-04} &	0.979 &	\sd{1.44e-04}\\
%         \bottomrule
%     \end{tabular}
%     \vspace{10pt}
%     \caption{Ablations.}
% \end{table}




==> compositional_ood_generalization/05_discussion.tex <==
\section{Discussion}\label{sec:discussion}

We presented a first step and a framework to study compositional generalization in a more principled way. Clearly, there remain many open questions and limitations that we leave for future work.

\paragraph{Supervised setting}
We only studied a supervised regression setting in which the model has access to the ground-truth latents of each training sample. Ultimately, we are
interested in the unsupervised setting akin to what is typically studied in identifiable representation learning. The unsupervised setting comes with inherent ambiguities that make generalizations guarantees harder to derive. Still, the results in this paper build an important foundation for future studies because sufficient conditions in the supervised setting can be considered necessary conditions in the unsupervised setting.

\paragraph{Jacobian and initial point} The proof of Theorem~\ref{theorem} utilizes the Jacobian of the ground-truth model. We emphasize again that this construction is necessary only for the proof and does not mean that we require access to the data-generating processes' full Jacobian for training.
%We merely need the Jacobian of $\boldsymbol C$ with respect to $\boldsymbol \varphi$ to determine how the sufficient support should be chosen, but this is trivial since $\boldsymbol C$ is assumed to be known.
Similarly, the existence of an initial point $\boldsymbol{p^0}$ is a technicality of the proof that is not reflected in the experiments. While it is not yet clear whether it is possible to complete the proof without the initial point condition,  we believe there is a self-consistency condition that might alleviate the need for this condition. The experiments thus hint at the existence of alternative proof strategies with relaxed assumptions.

\paragraph{Known composition function}
We also assume the composition function to be known which is approximately true in many interesting scenarios, such as object composition in scenes or the composition of instruments in music. In fact, many structured representation learning approaches like \eg SlotAttention~\cite{locatelloObjectCentricLearningSlot2020} incorporate structural components that are meant to mimic the compositional nature of the ground-truth-generating process. In other interesting cases like language, however, the composition function is unknown a priori and needs to be learned. This might be possible by observing how the gradients of $\boldsymbol{C}$ change with respect to a fixed slot, at least if certain regularity conditions are fulfilled. 

% \paragraph{Uniqueness of compositional representation}
% As explained in section~\ref{sec:compositionality}, there is no unique compositional representation for a given latent variable model. For our results to hold, there must be at least one compositional representation for which the compositional function $\boldsymbol{C}$ is known and for which the conditions outlined in Theorem \ref{theorem} are fulfilled.

% \paragraph{Shared component functions}
% Throughout this work we assumed an abstract setting in which each component function is different. In many scenarios, including our running dSprites example, each component is generated by the same function $\boldsymbol{\varphi}$. This substantially simplifies the problem and allows for much smaller sufficient supports $P$.

% \paragraph{Reference point}
% One technical point in Theorem \ref{theorem} is the need for a reference point, i.e. a point $\boldsymbol{p^0}$ for which the output of the component functions $\boldsymbol{\varphi_k(\boldsymbol{p^0})}$ is assumed to be known. While we so far cannot prove it, we believe there is a self-consistency condition that alleviates the need for a reference point. In none of our practical experiments we assumed a reference point and were still able to perfectly generalize compositionally. We leave a more formal treatment of this observation to future work.

\paragraph{Inductive biases}
Some of the conditions we derived can be relaxed in the presence of certain inductive biases. For example, models with an inductive bias towards shift invariance might be able to cope with certain gaps in the training support (e.g., if sprites are not visible in every position). Similarly, assuming all component functions $\boldsymbol{\varphi}$ to be identical would substantially simplify the problem and allow for much smaller sufficient supports $P$. The conditions we derived do not assume any inductive bias but are meant to formally guarantee compositional generalization. We expect that our conditions generalize to more realistic conditions as long as the core aspects are fulfilled.

\paragraph{Error bounds} Our generalization results hold only if the learned model perfectly matches the ground-truth model on the training distribution. This is similar to identifiable representation learning, where a model must find the global minimum of a certain loss or reconstruction error for the theory to hold. Nonetheless, extending our results towards generalization errors that are bounded by the error on the training distribution is an important avenue for future work.

\paragraph{Broader impact} Compositional generalization, once achieved, has the potential to be beneficial in many downstream applications. By substantially increasing sample and training efficiency, it could help to democratize the development and research of large-scale models. Better generalization capabilities could also increase the reliability and robustness of models but may amplify existing biases and inequalities in the data by generalizing them and hinder our ability to interpret and certify a model's decisions. 
% We thus caution against the blind application of compositional methods to any domain or context. 

% While we hope to have provided a flexible framework to study compositional generalization, there remain some clear limitations that we leave for future work. 
% only regression setting, not an inference setting
% setting still relevant because many structured learning methods like SlotAttention employ a structured decoder that should effectively learn to mimic the ground-truth generating process
% The first and most obvious shortcoming is that we can currently only make theoretical guarantees for a regression setting. In an unsupervised learning setup, comparisons to the ground-truth data-generating process come with inherent ambiguities, which make generalizations guarantees harder to derive. This is tied to the fact that we can only give generalization guarantees if the ground-truth function was fit perfectly to begin with. Extending our theory to incorporate error bounds should be the clear next step. Even so, we believe the setting studied in this paper to remain relevant, as many structured representation learning approaches like \eg SlotAttention~\cite{} incorporate inductive biases that heavily influence learning to mimic the ground-truth generating process. Generalization failure of these models remains an open problem.

% inductive biases
% At the same time, there are inductive biases in our framework that we are yet to explore. At the moment, we require the composition function $\boldsymbol C$ to be fully known, which limits the applicability of our theory. Relaxing the information that needs to be provided for $\boldsymbol C$ should also be a step towards fully unsupervised learning. On the other hand, an inductive bias that we have not employed so far is the assumption that all component functions $\boldsymbol{\varphi}$ are identical. This is a reasonable assumption in many settings that could help to further weaken the sufficient conditions stated here.

\section{Conclusion}

Machine learning, despite all recent breakthroughs, still struggles with generalization. Taking advantage of the basic building blocks that compose our visual world and our languages remains unique to human cognition. %We believe that overcoming this gap will require new learning approaches that go beyond the simple statistical learning strategies employed widely today.
We believe that progress towards more generalizable machine learning is hampered by a lack of a formal understanding of how generalization can occur. This paper focuses on compositional generalization and provides a precise mathematical framework to study it. We derive a set of sufficient conditions under which compositional generalization can occur and which cover a wide range of existing approaches. We see this work as a stepping stone towards identifiable representation learning techniques that can provably infer and leverage the compositional structure of the data. It is certainly still a long road toward scalable empirical learning techniques that can fully leverage the compositional nature of our world. However, once achieved, there is an opportunity for drastically more sample-efficient, robust, and human-aligned machine learning models.

==> compositional_ood_generalization/06_broader_impact.tex <==
\section*{Broader Impact}

==> compositional_ood_generalization/97_acknowledgements.tex <==
\section*{Acknowledgments}
We would like to thank (in alphabetical order): Jack Brady, Simon Buchholz, Attila Juhos, and Roland Zimmermann for helpful discussions and feedback.

This work was supported by the German Federal Ministry of Education and Research (BMBF): Tübingen AI Center, FKZ: 01IS18039A. WB acknowledges financial support via an Emmy Noether Grant funded by the German Research Foundation (DFG) under grant no. BR 6382/1-1 and via the Open Philantropy Foundation funded by the Good Ventures Foundation. WB is a member of the Machine Learning Cluster of Excellence, EXC number 2064/1 – Project number 390727645. This research utilized compute resources at the Tübingen Machine Learning Cloud, DFG FKZ INST 37/1057-1 FUGG. We thank the International Max Planck Research School for Intelligent Systems (IMPRS-IS) for supporting TW and PM.

==> compositional_ood_generalization/98_contributions.tex <==
\section*{Author contributions}
The project was led and coordinated by TW. TW and PM jointly developed the theory with insights from WB. TW implemented and conducted the experiments with input from PM and WB. TW led the writing of the manuscript with help from WB, PM, and MB. TW created all figures with comments from PM and WB.

==> compositional_ood_generalization/figs/function_class.tex <==
\begin{tikzpicture}
    % nodes
    \begin{scope}[minimum size=9mm, inner sep=0]
      \node[circle, fill=lightgray](z1) at (0, 3) {$\boldsymbol z_1$};
      \node[circle, fill=lightgray](z2) at (0, 1.8) {$\boldsymbol z_2$};
      \node[circle, fill=lightgray](zK) at (0, 0) {$\boldsymbol z_K$};

      \node[circle, fill=lightgray](zt1) at (3, 3) {$\boldsymbol{\tilde x}_1$};
      \node[circle, fill=lightgray](zt2) at (3, 1.8) {$\boldsymbol{\tilde x}_2$};
      \node[circle, fill=lightgray](ztK) at (3, 0) {$\boldsymbol{\tilde x}_K$};

      \coordinate(C) at (5, 1.5);
      \node[circle, fill=lightgray](x) at (6, 1.5) {$\boldsymbol{x}$};
    \end{scope}

    \node at (1.5, 1.15){$\vdots$};

    % edges
    \begin{scope}[out=0, in=180, line width=1pt]
        \draw (z1) edge[-latex] node[above]{$\boldsymbol \varphi_1$} (zt1) (zt1) edge (C);
        \draw (z2) edge[-latex] node[above]{$\boldsymbol \varphi_2$} (zt2) (zt2) edge (C);
        \draw (zK) edge[-latex] node[above]{$\boldsymbol \varphi_K$} (ztK) (ztK) edge (C);
        \draw (C) edge[-latex] node[above, pos=0]{$\boldsymbol C$}(x);
    \end{scope}
\end{tikzpicture}
